Preserving Privacy and Security in Federated Learning

Federated learning is known to be vulnerable to both security and privacy issues. Existing research has focused either on preventing poisoning attacks from users or on concealing the local model updates from the server, but not both. However, integrating these two lines of research remains a crucial challenge since they often conflict with one another with respect to the threat model. In this work, we develop a principle framework that offers both privacy guarantees for users and detection against poisoning attacks from them. With a new threat model that includes both an honest-but-curious server and malicious users, we first propose a secure aggregation protocol using homomorphic encryption for the server to combine local model updates in a private manner. Then, a zero-knowledge proof protocol is leveraged to shift the task of detecting attacks in the local models from the server to the users. The key observation here is that the server no longer needs access to the local models for attack detection. Therefore, our framework enables the central server to identify poisoned model updates without violating the privacy guarantees of secure aggregation.

==> macros.tex <==
% page size parameters
\usepackage{latexsym,setspace,xspace}
\setlength\itemindent{0.1in}
\setlength{\itemsep}{0in}

\setlength\topmargin{-0.75in}
\setlength\oddsidemargin{0.0in}
\setlength\evensidemargin{0.0in}
\setlength\parindent{0.0in} 
\setlength\textwidth{6.5in}
\setlength\textheight{9.25in}
\setlength{\parskip}{\medskipamount}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{3pt}%
\setlength{\belowdisplayshortskip}{3pt} }{\end{displaymath}}


% header hackery

\newlength{\toppush}
\setlength{\toppush}{2\headheight}
\addtolength{\toppush}{\headsep}


%\def\subjnum{CS 4/585}
%\def\subjname{Cryptography}

%\def\doheading#1#2#3{\vfill\eject\vspace*{-\toppush}%
%\vbox{\hbox to\textwidth{{\bf}\subjnum: \subjname \hfil Handout #1\strut}%
%\hbox to\textwidth{PSU --- Tom Shrimpton\hfil#3\strut}%
 %s   \hrule}}

\newcommand{\htitle}[1]{\vspace*{3.25ex}%
  \begin{center}{\Large\bf #1}\end{center}}


% page style that displays just footers
\makeatletter
\def\ps@justfooters{\let\@mkboth\@gobbletwo\def\@oddhead{}%
	\def\evenhead{}}
\makeatother

% \handout{handout label}{title}{date}

\newcommand{\handout}[3]{\thispagestyle{justfooters}%
  \markboth{\subjnum\ Handout \protect\ref{#1}: #2}%
    {\subjnum\ Handout \protect\ref{#1}: #2}%
  \pagestyle{myheadings}%
  \doheading{\protect\ref{#1}}{#2}{#3}%
  \htitle{#2}}

\newcommand{\procfont}[1]{\textbf{#1}}
\newcommand{\nfont}[1]{{\footnotesize #1}}


\newcommand{\dash}{{\mbox{-}}}
\newcommand{\taglen}{{\tau}}
\newcommand{\Pad}{P}
\newcommand{\Ctr}{{S}}

\newcommand{\outputs}{\Rightarrow}
\newcommand{\prf}{\mathrm{prf}}
\newcommand{\prp}{\mathrm{prp}}
\newcommand{\tprp}{\mathrm{tprp}}
\newcommand{\sprp} {{\pm\mathrm{prp}}}
\newcommand{\stprp}{{\pm\mathrm{tprp}}}
\newcommand{\ind} {{\mathrm{ind\mbox{-}{cpa}}}}
\newcommand{\auth} {{\mathrm{auth}}}
\newcommand{\indr}{{\mathrm{ind\$\mbox{-}{cpa}}}}
\newcommand{\indrcca}{{\mathrm{ind\$\mbox{-}{cca}}}}
\newcommand{\indcca}{{\mathrm{ind\mbox{-}{cca2}}}}
\newcommand{\nmcca}{{\mathrm{nm\mbox{-}cca}}}

\newcommand{\xxx}{{\mathrm{xxx}}}
\newcommand{\Encrypt}{\mathrm{Encrypt}}
\newcommand{\Decrypt}{\mathrm{Decrypt}}

\newcommand{\ERROR}{{\textsc{Error}}}
\newcommand{\invalid}{{\textsc{Invalid}}}

\newcommand{\CBC}{\mathrm{CBC}}
\newcommand{\CTR}{\mathrm{CTR}}
\newcommand{\CT}{{\mathit{CT}}}

\newcommand{\captionfont}{\small\sf }

\newcommand{\sep}{\:}
\newcommand{\kwfont}{\bf}
\newcommand{\AND}{\mbox{\kwfont and}}
\newcommand{\ALGORITHM}{\mbox{\kwfont Algorithm}}
\newcommand{\BEGIN}{\mbox{\kwfont begin}}
\newcommand{\DO}{\mbox{\kwfont do}}
\newcommand{\ELSE}{\mbox{\kwfont else}}
\newcommand{\END}{\mbox{\kwfont end}}
\newcommand{\FOR}{\mbox{\kwfont for}}
\newcommand{\IF}{\mbox{\kwfont if}}
\newcommand{\RETURN}{\mbox{\kwfont return}}
\newcommand{\THEN}{\mbox{\kwfont then}}
\newcommand{\TO}{\mbox{\kwfont to}}

\newcommand{\ZERO}{{\textbf{0}}}
\newcommand{\ONE}{{\textbf{1}}}
\newcommand{\error}{\mbox{\sc error}}
\newcommand{\true}{{\mathtt{true}}}
\newcommand{\false}{{\mathtt{false}}}
\newcommand{\undef}{{\textsc{undefined}}}
\newcommand{\dotdot}{{\,..\,}}
\newcommand{\xor}{{\,\oplus\,}}
\newcommand{\bits}{{\{0,1\}}}
\newcommand{\bitss}{\bits^*}
\newcommand{\e}{{\epsilon}}
\newcommand{\outputlen}{\varsigma}

\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}



% ====================================================================

% Theorem environments

\newtheorem{thm}{Theorem} %[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{propo}[thm]{Proposition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{assm}[thm]{Assumption}
\newtheorem{clm}[thm]{Claim}
\newtheorem{rem}[thm]{Remark}

\newenvironment{theorem}{\begin{thm}\begin{sl}}%
{\end{sl}\end{thm}}
\newenvironment{lemma}{\begin{lem}\begin{sl}}%
{\end{sl}\end{lem}}
\newenvironment{corollary}{\begin{cor}\begin{sl}}%
{\end{sl}\end{cor}}
\newenvironment{proposition}{\begin{propo}\begin{sl}}%
{\end{sl}\end{propo}}
\newenvironment{definition}{\begin{defn}\begin{em}}%
{\end{em}\end{defn}}
\newenvironment{assumption}{\begin{assm}\begin{em}}%
{\end{em}\end{assm}}
\newenvironment{claim}{\begin{clm}\begin{sl}}%
{\end{sl}\end{clm}}
\newenvironment{remark}{\begin{rem}\begin{em}}%
{\end{em}\end{rem}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\apref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\prref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{(\ref{#1})}}
\newcommand{\maybespace}{{\ifnum\springer=0{{\ }}\fi}}


\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
% deluxe proof environment
\def\qsym{\vrule width0.6ex height1em depth0ex}
\newcount\proofqeded
\newcount\proofended
\def\qed{ {\hspace{5pt}\rule[-1pt]{3pt}{9pt}}
\end{rm}\addtolength{\parskip}{-0pt}
\setlength{\parindent}{\saveparindent}
\global\advance\proofqeded by 1 }

\newenvironment{proof}%
 {\proofstart}%
 {\ifnum\proofqeded=\proofended\qed\fi \global\advance\proofended by 1
  \medskip}
\makeatletter
\def\proofstart{\@ifnextchar[{\@oprf}{\@nprf}}
\def\@oprf[#1]{\begin{rm}\protect\vspace{6pt}\noindent{\bf Proof of #1:\
}%
\addtolength{\parskip}{5pt}\setlength{\parindent}{0pt}}
\def\@nprf{\begin{rm}\protect\vspace{6pt}\noindent{\bf Proof:\ }%
\addtolength{\parskip}{5pt}\setlength{\parindent}{0pt}}

% ========================================================================

% Lists

\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=18pt%
\labelsep=7pt \leftmargin=25pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

\newenvironment{bignewenum}{%
\begin{list}{{\bf (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=18pt%
\labelsep=7pt \leftmargin=25pt \topsep=6pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{6pt} }}{\end{list}}

\newenvironment{tiret}{%
\begin{list}{\hspace{2pt}\rule[0.5ex]{6pt}{1pt}\hfill}{\labelwidth=18pt%
\labelsep=7pt \leftmargin=25pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{1pt} }}{\end{list}}

\newenvironment{onelist}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=15pt%
\labelsep=2pt \leftmargin=17pt \topsep=1pt% 
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{0pt} }}{\end{list}} 

\newenvironment{twolist}{%
\begin{list}{{\rm (\arabic{ctr}.\arabic{ectr})}%
\hfill}{\usecounter{ctr} \labelwidth=37pt%
\labelsep=7pt \leftmargin=44pt \topsep=0pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{0pt} }}{\end{list}}

\newenvironment{newitemize}{%
\begin{list}{$\bullet$}{\labelwidth=19pt%
\labelsep=7pt \leftmargin=26pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}

% =========================================================================

% General

\newlength{\savejot}
\setlength{\savejot}{\jot}


\newcommand{\heading}[1]{{\vspace{10pt}\noindent{\textsc{#1}}}}
\newcommand{\noskipheading}[1]{{\noindent{\textsc{#1}}}}

\newcommand{\headingg}[1]{{\textsc{#1}}}
\newcommand{\Heading}[1]{{\vspace{8pt}\noindent\textbf{#1}}}

\newcommand{\emptystring}{\varepsilon}
\newcommand{\concat}{\:\|\:}
\newcommand{\Concat}{\;\|\;}
\newcommand{\Colon}{{\,:\;\,}}

\newcommand{\N}{{{\sf N}}}
\newcommand{\R}{{{\rm\bf R}}}
\newcommand{\Y}{{{\sf Y}}}
\newcommand{\Z}{{{Z}}}

\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calT}{{\cal T}}

\newcommand{\D}{{\calD}}
\newcommand{\E}{{\calE}}
\newcommand{\K}{{\calK}}
\newcommand{\I}{{\calI}}
\renewcommand{\R}{{\calR}}
\renewcommand{\O}{{\calO}}
\newcommand{\M}{{\mathsf{Message}}}
\newcommand{\C}{{\mathsf{Ciphertext}}}


\newcommand{\Key}{\mathsf{Key}}
\newcommand{\IVspace}{\mathsf{IV}}
\newcommand{\Nonce}{\mathsf{Nonce}}
\newcommand{\Plaintext}{\mathsf{Plaintext}}
\newcommand{\Ciphertext}{\mathsf{Ciphertext}}

\newcommand{\goesto}{{\rightarrow}}
\newcommand{\eqdef}{\stackrel{\rm def}{=}}
\newcommand{\getsr}{{\:\stackrel{{\scriptscriptstyle \hspace{0.2em}\$}} {\leftarrow}\:}}
\newcommand{\getsd}{{\:\stackrel{{\scriptscriptstyle \hspace{0.2em}D}} {\leftarrow}\:}}
% \renewcommand{\choose}[2]{{{#1}\atopwithdelims(){#2}}}
\newcommand{\abs}[1]{{\displaystyle \left| {#1} \right| }}
\newcommand{\EE}[1]{{\E\left[{#1}\right]}}

\newcommand{\Damgard}{{\mbox{Damg{\aa}rd}}}

\newcommand{\strtonum}[1]{{ \mathsf{str2num}\left({#1}\right) }}
\newcommand{\numtostr}[2]{{ \mathsf{num2str}_{\scriptscriptstyle #2} 
                              \left( {#1} \right) }}

\newcommand{\Adv}{{\mathbf{\bf Adv}}}

\newcommand{\Randword}{\mathrm{Rand}}
\newcommand{\Permword}{\mathrm{Perm}}
\newcommand{\Randd}[2]{\ensuremath{\Randword({#1},{#2})}}
\newcommand{\Rand}[1]{\ensuremath{\Randword({#1})}}
\newcommand{\Rn}{{\calR_n}}
\newcommand{\Pn}{{\calP_n}}
\newcommand{\Perm}[1]{\ensuremath{\Permword({#1})}}
\newcommand{\Permm}[2]{\ensuremath{\Permword({#1},{#2})}}

\newcommand{\GF}{{\mathrm{GF}}}

\newcommand{\code}[1]{{\langle{#1}\rangle}}

\newcommand{\then}{{;\;}}
\newcommand{\andthen}{{\::\;\;}}

\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
\newcommand{\adv}{\ensuremath{\mathrm{Adv}}}
\newcommand{\hdir}{\mbox{\vspace{6mm}\~{ }}}



% ========================================================================

\makeatletter
% from  /usr/local/lib/tex/inputs/article.sty  and
%       /usr/local/lib/tex/inputs/latex.tex

\newcommand{\imply}{\boldmath{\Rightarrow}}

\newcommand{\IV}{{V}}

\newcommand{\CBCexplicitIV} {{\mathrm{CBC }}}
\newcommand{\CBCrandomIV}   {{\mathrm{CBC \$   }}}
\newcommand{\CBCencipherIVone} {{\mathrm{CBC 1}}}
\newcommand{\CBCencipherIVtwo} {{\mathrm{CBC 2}}}
\newcommand{\CBCencipherIVtwox} {{\mathrm{CBC 2 X}}}

\newcommand{\simulate}[3]{{\mbox{\textsl{SimulateOracles}}(#1,#2,#3)}}
\renewcommand{\Y}{{\cal Y}}
\newcommand{\setinvalid}{\mathrm{Invalid}}
\newcommand{\X}{{\cal X}}
\newcommand{\range}{\mathrm{Range}}
\newcommand{\domain}{\mathrm{Domain}}
\newcommand{\ran}{\mathrm{Range}}
\newcommand{\dom}{\domain}
\newcommand{\gamef}{\mathrm{GameF}}
\newcommand{\gamer}{\mathrm{Game\$}}
\newcommand{\cran}{\overline{\range}}
\newcommand{\cdom}{\overline{\domain}}
\newcommand{\bad}{\mathit{bad}}

\newcommand{\PrK}{{\mbox{$\Pr_K$}}}
\newcommand{\PrF}{{\mbox{$\Pr_F$}}}
\newcommand{\Bad}{{\mathsf{BAD}}}

\newcommand{\ctr}{\mathrm{CTR}}
\newcommand{\ctrFE}{{\ctr[F \times E]}}
\newcommand{\ctrRE}{{\ctr[{\cal R}_1 \times E]}}
\newcommand{\ctrRR}{{\ctr[{\cal R}_1 \times {\cal R}_2]}}
\newcommand{\KeyE}{\Key_E}
\newcommand{\KeyF}{\Key_F}
\newcommand{\TimeX}{\mathrm{Time}}
\newcommand{\authh}{{\mathrm{auth}*}}
\newcommand{\LAND}{{\;\wedge\;}}


\newcommand{\gamesfontsize}{\footnotesize}


\newcommand{\soln}[1]{\vspace*{1ex}\fbox{\begin{minipage}[c]{6.0in}{\textbf{\textit{Solution.}}\/#1}\end{minipage}} \vspace*{1ex}}


\newcommand{\mpage}[2]{\begin{minipage}{#1\textwidth}\gamesfontsize #2 \end{minipage}}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}{#1\textwidth}\gamesfontsize #2 \end{minipage}}}

\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
		\begin{tabular}{c@{\hspace*{.5em}}c}
		\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}} 
		&  
		\framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
		\end{tabular}
	}
\newcommand{\hfpagesss}[6]{
		\begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
		\framebox{\begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}} 
		&  
		\framebox{\begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}}
		&  
		\framebox{\begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}}
		\end{tabular}
	}


\def\codestretch{1.1}

\newcommand{\hpagesl}[3]{
	\begin{tabular}{c|c}
	  \begin{minipage}{#1\textwidth}\setstretch{\codestretch} #2 \end{minipage} 
	  & 
	  \begin{minipage}{#1\textwidth} #3 \end{minipage}
	\end{tabular}
	}

\newcommand{\hpagessl}[4]{
	\begin{tabular}{c|c}
	   \begin{minipage}[t]{#1\textwidth}\setstretch{\codestretch} #3 \end{minipage} 
	   & 
	   \begin{minipage}[t]{#2\textwidth}\setstretch{\codestretch} #4 \end{minipage}
	\end{tabular}
	}

\newcommand{\hpages}[3]{
	\begin{tabular}{cc}
	   \begin{minipage}[t]{#1\textwidth}\setstretch{\codestretch} #2 \end{minipage} 
	   & 
	   \begin{minipage}[t]{#1\textwidth}\setstretch{\codestretch} #3 \end{minipage}
	\end{tabular}
	}
\newcommand{\hpagess}[4]{
    \begin{tabular}{cc}
	   \begin{minipage}[t]{#1\textwidth}\setstretch{\codestretch} #3 \end{minipage} 
	   &
	   \begin{minipage}[t]{#2\textwidth}\setstretch{\codestretch} #4 \end{minipage} 
    \end{tabular}
	}

\newcommand{\hpagesss}[6]{
	\begin{tabular}{ccc}
	\begin{minipage}[t]{#1\textwidth}\setstretch{\codestretch} #4 \end{minipage} & 
	\begin{minipage}[t]{#2\textwidth}\setstretch{\codestretch} #5 \end{minipage} &
	\begin{minipage}[t]{#3\textwidth}\setstretch{\codestretch} #6 \end{minipage}
	\end{tabular}}
\newcommand{\hpagesssl}[6]{
	\begin{tabular}{c|c|c}
	\begin{minipage}[t]{#1\textwidth}\setstretch{\codestretch} #4 \end{minipage} & 
	\begin{minipage}[t]{#2\textwidth}\setstretch{\codestretch} #5 \end{minipage} &
	\begin{minipage}[t]{#3\textwidth}\setstretch{\codestretch} #6 \end{minipage}
	\end{tabular}}
\newcommand{\hpagessss}[8]{
	\begin{tabular}{cccc}
	\begin{minipage}[t]{#1\textwidth}\setstretch{\codestretch} #5 \end{minipage} & 
	\begin{minipage}[t]{#2\textwidth}\setstretch{\codestretch} #6 \end{minipage} &
	\begin{minipage}[t]{#3\textwidth}\setstretch{\codestretch} #7 \end{minipage}
	\begin{minipage}[t]{#4\textwidth}\setstretch{\codestretch} #8 \end{minipage}
	\end{tabular}}


\newcommand{\query}[1]{\procfont{query} {#1}:}
\newcommand{\queryl}[1]{\underline{\procfont{query} {#1}:}}
\newcommand{\oracle}[1]{\underline{\procfont{oracle} {#1}:}}
\newcommand{\oraclev}[1]{\underline{\procfont{oracle} {#1}:}\smallskip}
% \newcommand{\procedure}[1]{\underline{\procfont{procedure} {#1}:}}
\newcommand{\procedurev}[1]{\underline{\procfont{procedure} {#1}:}\smallskip}
\newcommand{\subroutine}[1]{\underline{\procfont{subroutine} {#1}:}}
\newcommand{\subroutinev}[1]{\underline{\procfont{subroutine} {#1}:}\smallskip}
\newcommand{\subroutinenl}[1]{{\procfont{subroutine} {#1}:}}
\newcommand{\subroutinenlv}[1]{{\procfont{subroutine} {#1}:}\smallskip}
\newcommand{\adversary}[1]{\underline{\procfont{adversary} {#1}:}}
\newcommand{\adversaryv}[1]{\underline{\procfont{adversary} {#1}:}\smallskip}
\newcommand{\experiment}[1]{\underline{{#1}}}
\newcommand{\experimentv}[1]{\underline{{#1}}\smallskip}


